Fides: Managing Data on Untrusted Infrastructure

Significant amounts of data are currently being stored and managed on third-party servers. It is impractical for many small scale enterprises to own their private datacenters, hence renting third-party servers is a viable solution for such businesses. But the increasing number of malicious attacks, both internal and external, as well as buggy software on third-party servers is causing clients to lose their trust in these external infrastructures. While small enterprises cannot avoid using external infrastructures, they need the right set of protocols to manage their data on untrusted infrastructures. In this paper, we propose TFCommit, a novel atomic commitment protocol that executes transactions on data stored across multiple untrusted servers. To our knowledge, TFCommit is the first atomic commitment protocol to execute transactions in an untrusted environment without using expensive Byzantine replication. Using TFCommit, we propose an auditable data management system, Fides, residing completely on untrustworthy infrastructure. As an auditable system, Fides guarantees the detection of potentially malicious failures occurring on untrusted servers using tamper-resistant logs with the support of cryptographic techniques. The experimental evaluation demonstrates the scalability and the relatively low overhead of our approach that allows executing transactions on untrusted infrastructure.

==> abstract.tex <==
\section{Abstract}
\label{sec:abs}

Significant amounts of data are currently
being stored and
managed on third-party servers. It is impractical
for many small scale enterprises to own their
private datacenters, hence renting third-party servers 
is a viable solution for such
businesses. But the increasing number 
of malicious attacks, both internal and external, 
as well as buggy software on third-party servers 
is causing clients to loose their trust
in these external infrastructures. While small
enterprises cannot avoid using external infrastructures, 
they need the right set of protocols to manage
their data on untrusted infrastructures.
In this paper, we propose \textit{\protocol},
a novel atomic commitment protocol that executes transactions
on data stored across multiple untrusted servers. To
our knowledge, \protocol is the first atomic commitment
protocol to execute transactions in an untrusted environment
without using expensive Byzantine replication.
Using \protocol, we propose
an {\em auditable} data management system, \textit{\system},
residing completely on untrustworthy infrastructure.
As an auditable system, \system guarantees
the detection of potentially malicious failures occurring on untrusted servers
using tamper-resistant logs with the support of cryptographic techniques.
The experimental evaluation demonstrates the scalability of our approach and the
relatively low overhead of executing transactions
on untrusted infrastructure.
%\noindent\textbf{Keywords}: Untrusted data management, 

==> blockchain_protocol.tex <==
\section{The \bblac Protocol}
\label{sec:b-blac}

Although \protocol gives us a mechanism to commit 
transactions in a byzantine environment, it has many
inherent limitations. Inspired by blockchain's techniques
on serial execution, handling concurrent requests and
tamper-proof logging, all this while inhibiting 
maliciousness, we propose an alternative to \protocol
that leverages permissioned blockchain called -- Byzantine 
Blockchain Atomic Commit (\bblac). \bblac's applicability
is similar to that of \protocol. At a high level both
protocols solve the same problem of byzantine atomic
commitment but the underlying details, the assumptions 
and the intrinsic limitations differ between the two.

\begin{figure}[th!]
\centering
 \includegraphics[scale=0.3]{figs/bblac.png}
\caption{\bblac system model.}
\label{fig:b-blac}
\end{figure}
\subsection{System Model}

While traditionally blockchains are used in the
paradigm of state machine replication (i.e., all 
nodes in the system maintain the same data), \bblac
uses blockchain to commit transactions across different
shards. Each shard maintains a disjoint set of data
items \textit{as well as} a replicated blockchain. 
Clients are non-malicious and generate transactions
consisting of
read-write operations on the data items stored across
one or more shards. Similar in concept to traditional
blockchains, certain details of every transaction 
is encapsulated in a block, which is then appended 
to the blockchain. But unlike traditional blockchains,
each block does \textbf{not} contain the actual 
transaction (the exact structure of the block will be 
discussed in the subsequent section). Since shard-servers
can fail maliciously, the shards run PBFT[cite]
to obtain consensus on the next block.
This restricts the number of malicious faults that can
be tolerated to less that $\frac{1}{3}$ of the shards
i.e., to tolerate $f$ failures, overall network should
have at least $3f+1$ shards. Similar to PBFT, although
the network can be asynchronous, certain preset time
bounds are assumed to provide liveness.

% We leverage the fact that PBFT 
% guarantees agreement on one single value (transaction)
% to commit one transaction at a time, even in the
% presence of contending transactions, nullifying the
% need for a shard to abort contending transactions.
% This provides serializability guarantees. Since 
% consensus ensures serialized execution of transactions,
% shards do not need any concurrency control mechanism.

As the shards can fail maliciously, one cannot trust
the shards to run the concurrency control (which allows
only one out of multiple conflicting transactions to
go through) correctly. An atomic commit protocol
cannot guarantee correct isolation or detect incorrectness
in the concurrency layer. Hence, \bblac assumes that the
transactions are \textit{independent transactions} or
\textit{one-shot transactions}~\cite{stonebraker2007end}. 
One-shot transactions consists of operations that span 
multiple shards but there is only one operation per shard. 
This mitigates a shard from independently aborting a 
transaction due to contention, thus mitigating the
need for concurrency control.
Furthermore, \bblac requires each shard to maintain
multi-versioned data based on the transaction commit
timestamps.

In a permissioned blockchain setting such as [cite],
one can traverse the chain from the genesis block and
can verify the correctness of any given data item. This
is because the blockchain maintains the entire history
(including inserts, updates, and deletes of each item)
of all the data items present in the system. \bblac, on
the other hand, is
developed to access data that is either too large to be
stored in a blockchain (millions of tuples) or for shards
that do not want to share their entire data with each
other. Hence, \bblac should guarantee 
correctness of data (e.g., Alice is spending only the 
money she possesses) even if one cannot see the entire
history of every data item (e.g., how much money did 
Alice start with).

In order to verify data whose entire history is not
stored in the blockchain, we leverage data authentication
technique using MHT~\cite{merkle1989certified}. \bblac uses 
the authentication method explained in section~\ref{sub:mht}
which requires additional verification information per
transaction. In essence, every block in the blockchain
now consists of a client generated transaction details
along with the verification
object \vo for that transaction. Although the protocol is 
explained with blockchain consisting of one transaction per
block, in practice a block can hold multiple transactions 
and the respective $\mathcal{VO}$s. In the next section we 
describe how this information is used to atomically 
commit transactions.

An important note here is since a set of data items are
stored only at one shard i.e., the data items are not 
replicated, if a shard maliciously corrupts its data, 
\bblac guarantees only detectablilty and not recoverabilty
of the corrupted data.

\begin{table}[]
\centering
\begin{tabular}{ c | c }  
\rowcolor{LightCyan}
 \textit{\textbf{key}} & \textit{\textbf{description}} \\
\hline
\hline
 TxnId & commit timestamp of txn \\ 
 \rowcolor{Gray}
 R-W set & read-write set of txn \\  
 \vo & verification object of txn \\
 \rowcolor{Gray}
 $h$ & hash of previous block \\
\end{tabular}
\caption{Details stored in each block}
\label{tab:block}
\end{table}

\subsection{The protocol}

Algorithm~\ref{algo:bblac} presents a pseudo-code for the
working of \bblac protocol. As indicated in lines 1-4,
during initialization, each shard constructs a
MHT of the data tuples it is responsible for and shares
within a signed message
the MHT root with the other shards. Hence, the genesis
block i.e., the first block of the blockchain holds the
initial MHT roots of all the shards. These initial roots
are used as source of truth for each shard and data 
updated after each transaction can be authenticated
starting from the genesis block. 



\begin{algorithm}[h]
\caption{\bblac protocol}
\label{algo:bblac}
\begin{algorithmic}[1]

\State \textbf{init():}
\State \quad $blockchain \gets \{\}$
\State \quad $genesis\_block \gets init\_root_{S_i}$ \textbf{for each} shard $S_i$
\State \quad append $genesis\_block$ to $blockchain$
\newline
\State \textbf{upon receiving} $\mu = \big\langle end\_transaction(T_i)\big\rangle_{\sigma_c}$ request from client and
process is current PBFT leader \textbf{do}
\State \quad new block $b_i \gets$ [ $txnId$, \textit{R-W} set, empty \vo, $h_{i-1}$]
\State \quad send $\big\langle get\_VO(b_i, \mu)\big\rangle_{\sigma_L}$ to all shards involved in $T_i$
\newline
\State \textbf{upon receiving} $\big\langle get\_VO(b_i, \mu)\big\rangle_{\sigma_L}$ message and process is shard $S_k$ \textbf{do}
\State \quad  \textbf{if} message contains {\em valid signature} and $\mu$ \textbf{then}
\State \qquad construct \vo for tuples of $S_k$ in $T_i$ 
\State \qquad send $\big\langle VO(\mathcal{VO}, h_{b_i})\big\rangle_{\sigma_{Sk}}$ to the leader
\newline
\State \textbf{upon receiving} signed $VO$ messages from all involved shards and
process is current PBFT leader \textbf{do}
\State \quad concatenate the signed $VO$s and update $b_i$ 
\State \quad call \textbf{PBFT($b_i$)} to reach consensus on $b_i$
\newline
\State \textbf{upon} reaching consensus on $b_i$ \textbf{do}
\State \quad update state if shard was updated in $T_i$
\State \quad append $b_i$ to $blockchain$
\newline
\State \textbf{audit():}
\State \quad /* to audit a shard $S_k$ at time $ts \leq current\_time$ */
\State {\quad access the block committed at time $t \leq ts$ that 
\Statex \quad updated shard $S_k$}
\State \quad  based on the $R-W$ set stored in $b_i$, identify tuples \Statex \quad accessed from $S_k$. Obtain the values for those tuples \Statex \quad and $root_t$ from $S_k$.
\State \quad using the \vo stored in $b_i$ and $R-W$ values obtained \Statex \quad in previous step, compute expected $root_{t-S_k}$
\State \quad \textbf{if} $root_t \neq root_{t-S_k}$ \textbf{then}
\State \qquad data corruption detected at shard $S_k$

% \State \quad $expected\_roots = \{\}$
% \State \quad \textbf{for each} block $b_i = [T_i, \mathcal{VO}_{T_i}]$ in $blockchain$ \textbf{do}
% \State \qquad compute latest root for each shard $S_i$ using $b_i$
% \State \qquad $expected\_roots[S_i] \gets latest\_root_{S_i}$

% \State \quad \textbf{for each} shard $S_i$ \textbf{do}
% \State \qquad \textbf{if} $current\_root_{S_i} \neq  expected\_roots[S_i]$ \textbf{then}
% \State \qquad \quad data corruption detected at shard $S_i$
    
\end{algorithmic}
\end{algorithm}

Except for the genesis block, every block in the blockchain
stores the information shown in Table~\ref{tab:block} (if the
blocks contain more than one transaction, a list of the 
transaction details are stored per block). Each block has
a transaction id, which is the commit timestamp of that
transaction. Every shard versions its data based on this
timestamp. The block contains the read-write set i.e., the 
tuple ids (e.g., keys) of data items read or written by the
transaction. Additionally, blocks also contain the
verification object of the transaction (explained in more
detail below). Since the blockchain is a tamper-proof
log, each block also stores the hash of the previous block, 
forming a chain of blocks linked by their hashes. 
Thus, manipulation to one block will require manipulating
the rest of the chain.

When the client $c$ decides to end a transaction, it sends a
$\big\langle
end\_transaction(T_i)\big\rangle_{\sigma_c}$ request, where
$T_i$ is a unique string of $\langle client\_id, ts_i\rangle$,
$ts_i$ being the commit timestamp of the transaction. The
timestamp is assigned by the client rather than the leader
as the leader shard cannot
be trusted to assign correct timestamps. As shown in lines 5-8,
when the current PBFT view leader receives $\big\langle
end\_transaction(T_i)\big\rangle_{\sigma_c}$, it creates a new
block $b_i$ with \textit{txnId, R-W set}, an empty \vo and
hash $h$ of the previous block. The leader then sends
$\big\langle get\_VO(b_i, \mu)\big\rangle_{\sigma_L}$ to
all the shards involved in $T_i$ in order to collect the 
necessary $\mathcal{VO}$s. The leader also encapsulates
the client request as a proof. 

A shard $S_k$ responds to $get\_VO$ message by first 
validating the leader request as well as the encapsulated 
client request (lines 8-11).
It then constructs the \vo for the tuples 
of $S_k$ accessed in $T_i$. $S_k$ then encapsulates the
\vo along with the hash of the block $b_i$ it received
from the leader. The $txnId$ and $h_{i-1}$ present in
the block ties $S_k$'s \vo to the current transaction.
This is important because a malicious leader could 
rearrange the \vo of a benign shard for transaction $T_i$
in $T_{i+1}$ block, which could lead to an audit failure
of the shard. Hence, encapsulating $h_{b_i}$ within
the signed message, protects a correct shard from
a potential malign leader.

As indicated in lines 12-17 of the algorithm, the leader
waits till it receives the $VO$ messages from all the
involved shards. It then concatenates all the signed $VO$
messages (containing \vo and $h_{b_i}$) and updates the
block.  At this stage, if one or
more participating shards do not respond (due to crash,
network partition or intentional message drops), the leader
stops processing $T_i$ as an indication of aborting $T_i$.
A malicious leader could intentionally not process the
client request. To solve this, a client waits for certain
time to receive the response from the leader and if it
times-out, it sends the end transaction request to all the
shards (this is similar to PBFT). If the leader received
all the necessary responses, it triggers PBFT on block $b_i$.
Upon reaching consensus on $b_i$, all shards append $b_i$
to their copy of blockchain and the shards affected by $T_i$
update the tuples.

% \bblac uses a variant of PBFT called \textit{PBFTCommit} to
% reach consensus on the next block to be appended to the 
% blockchain. Note that PBFTCommit is run among a set of
% shards and not replicas. As shown in lines 5-8, when
% the current PBFT view leader receives $\big\langle
% end\_transaction(T_i)\big\rangle_{\sigma_c}$ request 
% from a client $c$, the leader assigns a commit 
% timestamp $ts_i$ to the transaction and creates a block
% $b_i$ with \textit{txnId, R-W set} and hash $h$ of the
% previous block.
% It then triggers PBFTCommit which is explained in 
% lines 9-28. As with PBFT, in the first phase, the leader
% shard sends a \textit{pre-prepare} message along with $b_i$. 
% As a response, all the other shards multicast a 
% \textit{prepare} message. If a shard $S_k$ contain tuples
% that are in the \textit{R-W set} of $T_i$, then $S_k$
% constructs
% the \vo for those tuples and sends it in the \textit{prepare}
% message. Every shard, upon receiving $2f$ prepare messages,
% first checks if all the shards involved in $T_i$ responded -
% if yes, the shard decides to commit $T_i$ along with 
% concatenating
% all the $\mathcal{VO}$s received and updates the block $b_i$.
% If a shard does not receive prepare message from one or more
% shards participating in $T_i$, the shard waits for a preset
% time interval before deciding to abort the transaction $T_i$;
% it updates the block with the decision and a partial or empty 
% \vo. Every shard then multicasts \textit{commit} message with
% the update block $b_i$. In the third phase, each shard waits
% for at least $2f+1$ commit messages and checks if all of them
% have \textsf{commit} decision; if yes, the shard updates
% the decision to \textsf{commit} (even if it had previously 
% decided to abort due to timeout) and \textsf{abort} otherwise.
% %The shard updates its block, if the decision differs. 
% It then appends $b_i$ to the blockchain, responds to the
% client and finally updates the data tuples versioned at time
% $ts_i$, if $T_i$ modified the tuples of that shard.


% Consider an example for PBFTCommit: if $T_1$ updates a
% data item $d_i$ in shard $S_1$
% and item $d_j$ in shard $S_2$, and the system has 4 shards
% ($f=1$), then during the \textit{prepare} phase, the prepare
% message of $S_1$ consists of $\mathcal{VO}(d_i)$, and similarly,
% $S_2$'s message consists of $\mathcal{VO}(d_j)$. If all
% shards received $2f$ prepares, including $S_1$ and $S_2$'s 
% prepares, then all shards decide to commit $T_1$ and concatenate 
% all $\mathcal{VO}$s and update the block $b_1$ before multicasting 
% it in the \textit{commit} phase. In the \textit{commit} phase,
% a shard waits for $2f+1$ commit messages and if all those
% messages has commit as decision, the shard updates its
% decision and responds to the client.

The serializability of contending transactions is guaranteed by 
achieving consensus on one block at a time. The verification
object stored in each block provides a way to authenticate
correct updates on disjoint data stored in each shard.
Although we describe storing one transaction per block for
ease of explanation, \bblac can be 
extended to hold multiple transactions and their 
respective verification objects in each block.

Lines 32-38 in the algorithm indicates an audit function. At
any point in time $ts \leq$ \textit{current time}, an auditor
$\mathcal{A}$ can decide to audit a shard, say $S_k$. To do so, 
$\mathcal{A}$ collects the blockchain (either by reading from
one shard of from $f+1$ shards) and fetches a block with
transaction $T_i$ that has \textit{R-W set} in $S_k$ and
with commit timestamp $t \leq ts$. From this block $\mathcal{A}$
knows the transaction decision, \textit{R-W set}, and the
corresponding \vo. The auditor then communicates with $S_k$
to obtain the values in \textit{R-W set} as well as the 
MHT root of $S_k$'s data at time $t$. Since the shards 
maintain multi-versioned data based on commit timestamps,
$S_k$ will respond with the data values accessed in $T_i$
and the MHT root at time $t$. The auditor, using the values
sent by $S_k$ and \vo stored in the block, computes the
expected MHT root and compares it with the one sent by
the shard. A mismatch indicates that either the shard 
never committed (or aborted) transaction $T_i$ or that 
it has corrupted the data. This detection is enabled
given that MHTs use one-way
hashing functions (i.e., $h(x) \neq h(y)$).

% As a simple example, consider that blockchain has only 
% three blocks: the genesis block , followed by 2 blocks
% with transactions $T_1$ and $T_2$, committed at time 
% $t_1$ and $t_2$ respectively. If $\mathcal{A}$ decides
% to audit shard $S_2$ and that $T_2$ was the last 
% transaction to modify $S_2$, $\mathcal{A}$ obtains block
% $b_2$ and asks $S_2$ for the values of tuple ids present 
% in $b_2$, as well the the MHT root of $S_2$'s data at
% time $t_2$. 

\subsection{Discussion}

This section discusses how \bblac solves some of the limitations
of \protocol protocol while also discussing some of its own
constraints.

\begin{itemize}
    \item \textit{Concurrency Control and Handling Concurrent 
    Transactions}: The restriction on one-shot transactions
    \cite{stonebraker2007end} obliterates the need and hence
    any 
    malicious behaviour at the concurrency control layer. The 
    use of byzantine consensus protocol, PBFTCommit, eliminates
    the issue with handling concurrent transactions that was 
    present in \protocol.
    %
    \item \textit{Audit-ability}: \bblac maintains a blockchain 
    to store information about transaction history, thus 
    creating a tamper-proof log stored at each shard. This 
    provides audit-ability.
    %
    \item \textit{Independent Aborts}: The serialized execution of 
    transactions eliminates the need for an explicit concurrency 
    control at each shard. This takes away the freedom from a 
    shard to independently abort a transaction. The only reason a
    transaction gets aborted is if a shard participating in that
    transaction has either crashed or been network-partitioned,
    thus being unable to produce \vo during commitment.
\end{itemize}

Limitations of \bblac over \protocol:
\begin{itemize}
    \item \textit{Upper-bound on failures}: As nodes in \bblac 
    leverage PBFT for agreement on the next block, 
    this restricts the number of shards that can fail maliciously
    to at most $f$ in a network of size $3f+1$. In comparison,
    \protocol guaranteed detect-ability as long as at least one 
    shard is failure-free (crash or byzantine).
    %
    \item \textit{Serial execution of transactions}: Restricting 
    the execution of one block at a time reduces the throughput of 
    \bblac as compared to \protocol which allows non-contending
    transactions to commit.
    %
    \item \textit{One-shot transactions}: Although we argued that
    one-shot transactions mitigates trust requirements at the
    concurrency control level, it is more restrictive than the
    more generalized kinds of transactions that can be used
    in \protocol. 
    
\end{itemize}

==> byz_commit.tex <==
\section{The \protocol protocol}
\label{sec:protocol}

% Although \bblac provides a way to atomically commit
% transactions under a byzantine failure model, using
% PBFT to reach consensus on a transaction poses stringent
% requirements on the number of tolerated failures $f$ and
% the total number of shards requires to tolerate $f$ 
% failures.
In this section, we propose a novel byzantine atomic
commit protocol, \protocol. \protocol utilizes MHT for data
verification and digital signatures for message 
authentication (section~\ref{sec:background}) to commit 
transactions across potentially malicious shards.
The failure model is motivated by Dolev and Strong's~\cite{dolev1983authenticated}
work where the unforgeability of digital signatures
allows the number of tolerated failures $f$ to be any 
number less than $n$, the total network size ($n>f$).
\protocol protocol is applicable in two scenarios: 1)
If an enterprise rents servers from multiple cloud
providers (e.g. Amazon AWS, Google GCP, Microsoft
Azure, etc.) and places different partitions or shards
of the data in servers spanning various providers. 
2) To develop applications comprising of different enterprises
that do not fully trust each other (e.g. supply-chain
management such as construction company and hardware
manufacturer). \protocol detects data corruption
(intentional or unintentional) for such applications
that produce transactions accessing data stored 
in one or more distrusted servers.

For ease of explanation, we present the \protocol protocol
in two different modes. The first mode is simpler but
has stronger assumptions
about a trusted, central coordinator that is orchestrating
transaction commitment. The second mode is less restrictive 
and is a fully decentralized byzantine atomic
commitment solution. Since a shard can fail 
maliciously and can potentially corrupt the data, 
\protocol can detect such a malicious behavior. More
precisely, if a shard $S$ corrupts its data after 
transaction $T_i$, the corruption will be detected while
committing transaction $T_{i+1}$, which then will be
aborted. 
% As we do not assume any replication, the protocol
% as is does not deal with recovering the corrupt data.

\input{system_model}
\input{centralized.tex}
\input{decentralized.tex}

==> centralized.tex <==
\subsection{Centralized solution}
\label{sub:centralized}

\begin{figure}[th!]
\centering
\includegraphics[scale=0.4]{figs/central.png}
\caption{\protocol centralized solution.}
\label{fig:centralized}
\end{figure}

\begin{algorithm}[h]
\caption{\protocol in centralized approach}
\label{algo:centralized}
\begin{algorithmic}[1]

\State \textbf{init():}
\State \quad \textbf{if} process is coordinator $\mathcal{C}$ \textbf{then}
\State \qquad \textbf{for each} shard $S_i$ \textbf{do}
\State \qquad \quad $last\_root_{S_i} \gets init\_root_{S_i}$ 


\State \textbf{upon receiving} \textit{end\_transaction($T_i$)} request from client and process is $\mathcal{C}$ \textbf{do}

\State    \qquad send $\big\langle get\_vote(T_i)\big\rangle_{\sigma_C}$ to all shards in $T_i$
    


\State \textbf{upon receiving} $\big\langle get\textunderscore vote(T_i)\big\rangle_{\sigma_C}$ from coordinator and process is shard $S_j$ \textbf{do}

\State    \quad \textbf{if} message contains {\em valid signature} \textbf{then}

\State    \qquad decide to \textsf{commit} or \textsf{abort} $T_i$
\State    \qquad $\mathcal{VO}_i \gets \textsf{null}$
\State    \qquad \textbf{if} $decision=\textsf{commit}$ \textbf{then}
\State    \qquad \quad construct $\mathcal{VO}_i$ for the tuples accessed in $T_i$
\State    \qquad send $\big\langle vote(decision, \mathcal{VO}_i, root_{i-1})\big\rangle_{\sigma_{S_j}}$ to $\mathcal{C}$

\State \textbf{upon receiving} votes from \textbf{all} the involved shards and process is coordinator \textbf{do}

\State \quad $final\_decision \gets \textsf{commit}$
\State \quad $corrupted\_shards \gets \{\}$
\State \quad \textbf{for each} shard $S_j$ \textbf{do}
\State \qquad fetch the last known root $last\_root_{S_j}$
\State   \qquad \textbf{if} $root_{i-1} \neq last\_root_{S_j}$ \textbf{then}
\State \qquad \quad $final\_decision \gets$ \textsf{abort}
\State \qquad \quad append $S_j$ to $corrupted\_shards$

\State   \qquad \textbf{else if} $decision=\textsf{abort}$ \textbf{then}
\State \qquad \quad $final\_decision \gets$ \textsf{abort}

\State \quad \textbf{if} $final\_decision=\textsf{commit}$ \textbf{then}
\State \qquad \textbf{update} $last\_root_{S_j}$ for each shard $S_j$
\State \quad send $\big\langle decision(T_i, final\_decision)\big\rangle_{\sigma_C}$ to all shards
    
\end{algorithmic}
\end{algorithm}

In this section, we develop a simplified version of the
\protocol commit protocol by using a centralized approach 
consisting of a coordinator driving the commitment. 
We assume the coordinator
to be trusted i.e., the coordinator process does not fail 
maliciously and only fails by crashing. We further 
assume that the coordinator is highly available
either using a master-shadow [cite] or replication [cite] 
technique. The centralized approach can be useful for small 
enterprises capable of hosting a small number of trusted 
coordinator(s) but are mostly outsourcing their data 
onto untrusted third party machines. 
%All transactions go through the coordinator.

Algorithm~\ref{algo:centralized} presents a pseudo-code 
for \protocol's centralized solution. At the genesis, 
each shard $S_i$ in the system constructs a MHT of its data 
and shares the initial MHT root, $init\_root_{S_i}$,
with the coordinator $\mathcal{C}$. $\mathcal{C}$
maintains the last known root, $last\_root_{S_i}$, for
each shard $S_i$ which is initialized with the $init\_root_{S_i}$
at the beginning, as shown in lines 1-4 of the algorithm.


Clients perform transactional read-writes on the data stored
across multiple shards. A client, upon completing the data access,
sends an 
\textit{end\_transaction($T_i$)} request to the coordinator 
$\mathcal{C}$ which triggers the transaction commitment.
Upon receiving the client request, as indicated in lines 5-6 of 
the algorithm, $\mathcal{C}$ sends a signed
$\big\langle get\_vote(T_i)\big\rangle_{\sigma_C}$ message 
to all the shards involved in transaction $T_i$.
The shards' response is indicated in lines 7-13.
The concurrency control in each shard
is responsible for maintaining the isolation level (e.g.
strict serializability, snapshot isolation, etc.) required
by  the application. Each shard $S_j$, based on the
underlying concurrency control mechanism it is using,
independently decides to either \textsf{commit} or
\textsf{abort} the transaction. 
Using the MHT constructed based on the latest data before 
$T_i$, the shard $S_j$ constructs the 
verification object $\mathcal{VO}_i$ (section~\ref{sub:mht}).
$\mathcal{VO}_i$ essentially consists of all the sibling 
nodes in the path from 
the tuples accessed in $T_i$ to the root of MHT. 
$S_j$ then responds to the coordinator with a signed
$\big\langle vote(decision, \mathcal{VO}_i,
root_{i-1})\big\rangle_{\sigma_{Sj}}$ message, where 
$root_{i-1}$ is the MHT root after the last committed 
transaction $T_{i-1}$.
The coordinator uses $\mathcal{VO}_i$ and $root_{i-1}$ to 
authenticate correct data updates.

The coordinator $\mathcal{C}$ waits until it receives votes 
from all the shards involved in $T_i$ and $\mathcal{C}$ 
performs verification using the responses before deciding
to commit or abort $T_i$. These steps are indicated 
in lines 14-26 of the algorithm. For now, assume $\mathcal{C}$
knows the last MHT root $last\_root_{S_j}$ after $T_{i-1}$ 
for every shard $S_j$ (we will
soon describe how $last\_root_{S_j}$ is computed by 
$\mathcal{C}$). The verification is done as 
follows: for each shard $S_j$, $\mathcal{C}$ retrieves its 
copy of the last known MHT root $last\_root_{S_j}$ 
%(initialized with $init\_root_{S_j}$) 
and compares it with $root_{i-1}$ sent by $S_j$ 
in the response message.  If $last\_root_{S_j}$ does
not match with the previous root $root_{i-1}$ sent by $S_j$,
this indicates that the data stored at $S_j$ has been 
manipulated between transactions $T_{i-1}$ and $T_i$, and thus,
$\mathcal{C}$ decides to abort $T_i$ along with appending
$S_j$ to the list of corrupted shards. On the other hand,
a non-malicious shard can genuinely decide to abort $T_i$ 
due to contention,
in which case $\mathcal{C}$ simply chooses to abort $T_i$. If
verification was successful \textbf{and} all shards decided to
commit $T_i$, $\mathcal{C}$ decides to commit the transaction
and sends a signed message containing the decision to all the
involved shards.


If $\mathcal{C}$ decides to commit $T_i$, $\mathcal{C}$ needs
to update the last known roots of the shards updated in $T_i$
so as to detect subsequent
data corruptions. For each shard $S_j$, $\mathcal{C}$ uses
the $\mathcal{VO}_i$ sent by $S_j$ and since $\mathcal{C}$
knows the tuple values updated in $T_i$, $\mathcal{C}$ constructs 
the MHT by hashing the updated values in $T_i$ and uses the 
sibling node information
present in $\mathcal{VO}_i$ to obtain the new $last\_root_{S_j}$.
For example, in Figure~\ref{fig:mht_ex},
if $T_i$ updated $a$'s value in shard $S_1$, $\mathcal{C}$
can compute $h(a)$ using the updated value in $T_i$ and
use $h_b$ from $\mathcal{VO}_i$ to further compute 
$h_{a,b} = h(h(a)|h(b))$ and finally used $h_{c,d}$ from 
$\mathcal{VO}_i$ to compute $last\_root_{S1}=h(h_{a,b} 
| h_{c,d})$.



During the commitment of the next transaction $T_{i+1}$,
the coordinator will use the updated $last\_root_{S_j}$ for shard $S_j$ 
to identify unauthorized data manipulation at $S_j$ between
transactions $T_i$ and $T_{i+1}$. If a malicious
shard $S_m$ corrupts a tuple value from $x$ to $y$ after 
transaction $T_i$ and before $T_{i+1}$, the only way this
can be undetected by $\mathcal{C}$ is if $h(x) = h(y)$, so
that the root remains unchanged. But since the premise
of \protocol assumes one-way hash functions (i.e., 
$h(x) \neq h(y)$), $S_m$'s manipulation will always be detected
by $\mathcal{C}$.





% we will assume that the coordinator is trusted and all transactions
% go through the coordinator. Upon receiving the ${end\_transaction(T_{i})}$ request
% from the client, the coordinator sends \textsf{get\_value($T_i$)} to all the involved shards.
% Each shard send a response tuple consisting of  $<$\textsf{commit} or \textsf{abort}, $\mathcal{VO}$, $root_{i-1}>$. The responses are signed by the shards. The coordinator
% verifies if $root_{i-1}$ sent by each shard matches the previous root that the coordinator
% had. The coordinator then decides to commit $T_i$ if all shards voted \textsf{commit},
% and abort if any \textit{one} of the shards voted \textsf{abort} and sends the decision 
% to the shards. The shards, as a response to the decision message, will update the data
% and compute the new root, $root_i$ and send it to the coordinator.
% Since the coordinator is aware of the keys updated in transaction $T_i$, and it collected
% all the $\mathcal{VO}$s from each shard, the coordinator will compute the expected $root_i$
% and ensure that the $root_i$ sent by each shard matches the expected hash.  

==> data_verification.tex <==
\subsection{Datastore Layer}
\label{sub:ds_layer}

The datastore stores a
set of data items and their
associated read and write
timestamps, indicating the commit timestamp 
of the last transaction
that read and wrote the data item, respectively. 
The datastore can be single-versioned or multi-versioned.
For multi-versioned datastores, when a transaction 
commits, the datastore layer additionally creates
a new version of the data items accessed in the
transaction while maintaining the older versions.
Although an application using \system can choose between
single-versioned
or multi-versioned data, multi-versioned data
can provide \textit{\textbf{recoverability}}.
If a failure occurs,
%\system identifies the exact version that failed;
the data can then be reset to the last sanitized 
version and the application can resume execution from 
there.

\textbf{Detecting Malicious Behavior}:
A correct
server updates the datastore for each committed
transaction: for single versioned datastores, the
latest state of data (data values and timestamps) is correct; 
for multi-versioned datastores, each version of the data 
is correct. However, a malicious
server can either completely omit the updates of a 
committed transaction or update the data incorrectly.


To detect data corruption, we use the data 
authentication technique proposed by
Merkle~\cite{merkle1989certified}
discussed in Section~\ref{sub:mht}. To identify data
corruption,
an auditor uses the information stored within each block:
the hashes of the values in the read and write sets
and the Merkle Hash Tree (MHT) roots. 

\textit{\textbf{Multi-versioned datastores:}}
For multi-versioned datastores, the audit 
policy can involve auditing a single version chosen 
arbitrarily or exhaustively auditing all versions
starting from either the first version
(block 0) or the latest version. We explain 
auditing a single version, which can easily be extended to
exhaustively auditing all versions.


Let $T_i$ be a transaction committed at timestamp
$ts$ that read and wrote data item $x$ 
stored in server $S_k$.
Assume the auditor audits server $S_k$ at version $ts$. Once the auditor
notifies the server about the audit,
the
server constructs the Merkle Hash Tree with the
data at version $ts$
as the leaves; $S_k$ then shares the 
\textit{Verification Object} \vo -- consisting of all
the sibling nodes along the path from the data $x$
to the root-- with the auditor.

The log entry corresponding to transaction $T_i$ 
stores the value read for item $x$ and the
new value written.
The auditor uses i) the \vo sent by $S_k$, and ii) the 
hash of $x$'s value stored in the write set of the log,
to compute the
expected MHT root for the data in $S_k$. The auditor
then compares the computed root with the one stored in 
the log. A mismatch indicates that the data at version
$ts$ is incorrect.

\textit{\textbf{Single-versioned datastores:}}
For single versioned data, the correctness is only with
respect to the latest state of the datastore. Hence,
rather than using an arbitrary block to obtain
the MHT root of server $S_k$, the auditor uses the latest
block in the log that accessed
the data in $S_k$ to obtain the latest MHT root. 
The other steps are similar to multi-versioned datastores: 
the auditor fetches the \vo based on the latest state 
of $S_k$ and recomputes
the MHT root to compare the root stored in the 
log. 

\vspace{0.5em}
\noindent\textbf{\textit{Lemma 5}}: If a malicious server 
corrupts the data it stores,
the auditor detects it. For multi-versioned datastore, the 
auditor
detects the precise version at which the data was corrupted.

\textit{\textbf{Proof}}:
Detection is guaranteed since Merkle Hash Trees (MHT) use
collision-free
hash functions (i.e., $h(x) \neq h(y)$ where $x \neq y$), and a malicious
server cannot update a data value such that the MHT root
stored in the block
matches the expected root computed by the auditor. 
% For
% single versioned datastores, the latest block in the log
% to access the data is used to extract the MHT
% root. 
For multi-versioned datastores, the auditor identifies
the precise version at which data corruption occurred 
by systematically authenticating all blocks in the log
until a 
version with mismatching MHT roots is detected.
\hfill$\Box$

==> decentralized.tex <==
\subsection{Decentralized solution}
\label{sub:decentralized}

\begin{figure}[th!]
\centering
\includegraphics[scale=0.4]{figs/decentral.png}
\caption{\protocol decentralized solution.}
\label{fig:decentralized}
\end{figure}

\begin{algorithm}[t]
\caption{\protocol in decentralized approach}
\label{algo:decentralized}
\begin{algorithmic}[1]

\State \textbf{init():}
\State \quad \textbf{for each} shard $S_i$ \textbf{do}
\State \qquad $last\_root_{S_i} \gets init\_root_{S_i}$ 


\State \textbf{upon receiving} $\mu = \big\langle end\_transaction(T_i)\big\rangle_{\sigma_c}$ request from client and process is shard $S_k$ \textbf{do}

\State    \qquad send $\big\langle get\_vote(T_i, \mu)\big\rangle_{\sigma_{S_k}}$ to all shards

\State \textbf{upon receiving} $\big\langle get\_vote(T_i, \mu)\big\rangle_{\sigma_{S_k}}$ from $S_k$ and process is shard $S_j$ including $S_k$ \textbf{do}

\State    \quad \textbf{if} message contains {\em valid signature} and $\mu$ \textbf{then}

\State    \qquad decide to \textsf{commit} or \textsf{abort} $T_i$
\State    \qquad $\mathcal{VO}_i \gets \textsf{null}$
\State    \qquad \textbf{if} $decision=\textsf{commit}$ \textbf{then}
\State    \qquad \quad construct $\mathcal{VO}_i$ for the tuples accessed in $T_i$
\State    \qquad send $\big\langle vote(decision, \mathcal{VO}_i, root_{i-1})\big\rangle_{\sigma_{S_j}}$ to all shards

\State \textbf{upon receiving} votes from \textbf{all} the involved shards and process is any shard $S_k$ involved in $T_i$ \textbf{do}

\State \quad $local\_decision \gets \textsf{commit}$
\State \quad $corrupted\_shards \gets \{\}$
\State \quad \textbf{for each} shard $S_j$ \textbf{do}
\State \qquad fetch the last known root $last\_root_{S_j}$
\State   \qquad \textbf{if} $root_{i-1} \neq last\_root_{S_j}$ \textbf{then}
\State \qquad \quad $local\_decision \gets$ \textsf{abort}
\State \qquad \quad append $S_j$ to $corrupted\_shards$

\State   \qquad \textbf{else if} $decision=\textsf{abort}$ \textbf{then}
\State \qquad \quad $local\_decision \gets$ \textsf{abort}

\State \quad \textbf{if} $local\_decision=\textsf{commit}$ \textbf{then}
\State \qquad \textbf{update} $last\_root_{S_j}$ for each shard $S_j$
\State \quad send $\big\langle decision(T_i, local\_decision)\big\rangle_{\sigma_{S_k}}$ to all shards

\State \textbf{upon receiving} $\big\langle decision(T_i, decision)\big\rangle_{\sigma_{S_k}}$ from all shards and process is any shard $S_j$ involved in $T_i$ \textbf{do}
\State \quad $final\_decision \gets local\_decision$
\State \quad \textbf{for each} shard $S_k$ \textbf{do}
\State \qquad \textbf{if} $decision_{S_k} \neq local\_decision_{S_j}$ \textbf{then}
\State \qquad \quad $final\_decision \gets \textsf{abort}$ 
\State \quad \textbf{if} $final\_decision = \textsf{commit}$ and $T_i$ updated $S_j$ \textbf{then}
\State \qquad update local state
\State \quad send $\big\langle reply(T_i, final\_decision)\big\rangle_{\sigma_{S_j}}$ to client
    
\end{algorithmic}
\end{algorithm}

The decentralized approach is less stringent on some of
the requirements of the centralized solution;
mainly there is no trusted, centralized coordinator to run
transaction commitment. Algorithm~\ref{algo:decentralized}
presents the pseudo-code for the decentralized \protocol 
protocol. Although the underlying data verification technique
is same as the centralized approach, the primary difference 
is that instead of only the coordinator verifying the 
transactions, here every shard performs verification. 
Removing the trusted component in a byzantine setting 
requires \textit{all-to-all} communication in place of
\textit{one-on-one} communication between the coordinator
and the shards, as well as an additional phase. 
% The all-to-all multicasts between the shards
% is necessary because 
The failure model assumes $n > f$ i.e.,
as long as at least one shard is benign and failure-free, 
a malicious fault will be detected and the particular 
shard(s) causing the failure will be identified. 
Although not explicitly mentioned in the
algorithm, all processes log the received messages along
with the signatures as a proof that can be used if a
node is being audited. \textbf{(Is the last sentence too vague?)}

As indicated in lines 1-4 of Algorithm~\ref{algo:decentralized},
every shard
initializes the last known root, $last\_root_{S_i}$, for
each shard $S_i$ in the system. A client can send
$\big\langle end\_transaction(T_i)\big\rangle_{\sigma_c}$ 
message to any of the shards participating in $T_i$.
When a shard $S_k$
receives a $\mu = \big\langle end\_transaction(T_i)
\big\rangle_{\sigma_c}$ request from a client $c$, 
$S_k$ sends a signed $\big\langle get\_vote(T_i, \mu)\big\rangle
_{\sigma_{S_k}}$ message to to not only the shards involved in 
$T_i$ but to all the shards in the system because we assume
at most $n-1$ out of $n$ shards can fail maliciously.
Note that the $get\_vote$ message also contains
the client's original request $\mu$ as a proof because 
$S_k$ could be maliciously sending $get\_vote$ requests to 
other shards.

As shown in lines 6-12 of the algorithm, all the shards
validate if the message and the encapsulated client
request $\mu$ contains valid signatures. Then, all the shards 
involved in $T_i$ (including $S_k$), respond
to the $get\_vote$ by independently deciding to either
\textsf{commit} or \textsf{abort} $T_i$ based on the 
concurrency control model used. If a shard locally 
decides to commit $T_i$, it constructs the verification
object for the tuples being accessed in $T_i$ and
\textbf{multicasts} its vote in $\big\langle vote(decision,
\mathcal{VO}_i, root_{i-1})\big\rangle_{\sigma_{S_j}}$
message to all the shards.

Each shard $S_k$ involved in $T_i$ waits until it receives all
the votes from the other shards. $S_k$ locally performs
data verification (which was done only at the coordinator
in the centralized approach) similar to Algorithm
\ref{algo:centralized}. $S_k$ fetches the last known 
MHT root for each shard and compares it with $root_{i-1}$
sent by the corresponding shard and if the two roots
mismatch, $S_k$ decides locally to abort the transaction and
notifies other shards along with the proof of the anomalous
behavior. $S_k$ also decides to abort $T_i$ if any shard in 
$T_i$ sent a vote with \textsf{abort} decision. $S_k$ then
multicasts $\big\langle decision(T_i, local\_decision)
\big\rangle_{\sigma_{S_k}}$ message to all the shards.

As there is no trust between the shards and a shard can
maliciously send \textsf{commit} $T_i$ for certain shards
and \textsf{abort} for some others, the decentralized 
approach requires another phase, as shown in lines 26-31.
In this phase a shard $S_j$ collects the $decision$ message
from all the shards and compares each of their decision
with its local decision. If there is a mismatch, then it
sends a final decision of \textsf{abort} in the
\textit{reply} message to the client,
along with piggybacking information such as
$corrupted\_nodes$ and the set of $votes$ it received
from the other shards, as a proof. If the local
decision matches with that of other shards, only
the final decision is sent the the \textit{reply}.
If the client receives conflicting final decisions for
the transaction $T_i$, it detects an anomaly and it can either
notify application owner or itself initiate any offline 
action to penalize and/or rectify the malicious behavior.  
% A client uses the piggybacked 
% information to identify particular misbehaving shard(s). 

If a shard, $S_n$ was not involved in $T_i$, it stores all the
messages (\textit{get\_vote, vote, decision}) until the
decision message is received from all the shards in $T_i$.
$S_n$ uses the \vo sent in the \textit{vote} message and
if $T_i$ is to be committed, $S_n$ updates the last known
roots for the shards updated in $T_i$. $S_n$ can also
verify if the $root_{i-1}$s sent by the shards in $T_i$
match the last known root at $S_n$ and if the verification
fails, it can trigger any offline corrective measure.
% In this approach, we do not assume a centralized, trusted coordinator. When the client
% intends to end the transaction, it sends ${end\_transaction(T_i)}$ to one of the involved
% shards in $T_i$. Let the shard chosen by the client be $\mathcal{C}$, which acts as
% a coordinator to commit the transaction. The only additional
% responsibility of  $\mathcal{C}$ is to trigger the commitment by sending
% \textsf{get\_value($T_i$)} to all the other shards accessed by $T_i$. 
% Any shard involved in transaction $T_i$, upon receiving the \textsf{get\_value($T_i$)}
% message will broadcast the response to \textit{all} the involved shards. The response
% will consist of a tuple $<$\textsf{commit} or \textsf{abort}, $\mathcal{VO}$, $root_{i-1}>$.
% Since all shards broadcast their decision to all the other shards, each shard can make the
% decision independently. Once a shard decides on the value, it updates the data and 
% broadcasts it's decision along with the new root, $root_i$ to all the other shards. Now,
% as long as there is at least one good node, an auditor can go through the logged 
% roots, $root_{i-1}$, along with transaction $T_i$ and the corresponding $\mathcal{VO}$ 
% object to verify if any shard has manipulated the data in a way that it was not supposed
% to.

\subsection{Limitations}

Having described the two variants of \protocol protocol, we now
discuss the limitations present in the protocol.
\begin{itemize}
    \item \textit{Concurrency Control}:  \protocol is oblivious to 
    the underlying concurrency control technique used
by the shards. If a shard is malicious at the CC level (either
due to a bug or intentional maliciousness), it can violate the 
serializability guarantees required at the application layer
by allowing
two contending transactions to commit. 
%
\item \textit{Independent aborts}: Since each shard is capable
of aborting transactions independently, a malicious shard could
abort every incoming transaction and stagnate the system.
%
\item \textit{Audit-ability}: The working of \protocol does not
require maintaining logs for past transactions, which prevents
an independent auditor to audit the system in the event of any
conflict.
%
\item \textit{Handling concurrent transactions}: 
This limitation is better illustrated as an example.
For simplicity, 
consider the centralized approach and consider two concurrent
non-contending (accessing disjoint tuples) transactions,
$T_1$ and $T_2$ modifying shard 
$S_1$. The coordinator sent decision for $T_1$ first followed by
$T_2$ and updates the expected root of $S_1$ after $T_2$.
But due to the 
asynchronous network, $S_1$ could receive the decisions in 
the reverse order and update its root based on $T_1$. Now the 
expected root and the actual root of $S_1$ will not match and 
the coordinator may suspect $S_1$ of data corruption. Solving
this will require storing of all potential roots based on
concurrent transactions at the coordinator
and logging the signed messages in the order they arrived at the
shard, both of which are complex solutions.
\end{itemize}

In the following section, we develop a blockchain based 
protocol that addresses some of the limitations of \protocol.



